Efficient and Optimal Algorithms for Contextual Dueling Bandits under Realizability

We study the $K$-armed contextual dueling bandit problem, a sequential decision making setting in which the learner uses contextual information to make two decisions, but only observes \emph{preference-based feedback} suggesting that one decision was better than the other. We focus on the regret minimization problem under realizability, where the feedback is generated by a pairwise preference matrix that is well-specified by a given function class $\mathcal F$. We provide a new algorithm that achieves the optimal regret rate for a new notion of best response regret, which is a strictly stronger performance measure than those considered in prior works. The algorithm is also computationally efficient, running in polynomial time assuming access to an online oracle for square loss regression over $\mathcal F$. This resolves an open problem of Dud\'ik et al. [2015] on oracle efficient, regret-optimal algorithms for contextual dueling bandits.

==> genf.tex <==
\section{Main Results: Algorithm and Analysis for General Function Classes $\cF$}
\label{sec:genf}

In this section we address the most general setup  for any arbitrary function class $\cF$. Towards this we first analyze the min-max optimality of the problem which lead to an efficient $O(\sqrt{\regsq(T)KT})$ algorithm assuming access to an \emph{online regression oracle} \oreg\, (details in Sec. \ref{sec:oreg}). {This resolves the open problem of finding a computationally efficient and near-optimal $\tO(\sqrt T)$ algorithm for general contextual dueling bandit problem (as discussed in Sec. \ref{sec:intro})}.
\vspace{-10pt}

\subsection{Development of \algf: Min-Max Optimal Best-Response Regret Analysis}
\label{sec:minmax}

Towards bounding the $T$ step cumulative regret, we try to analyze the following `minimax value' per round: 
Assuming the learner plays $(a_t,b_t) \sim \p_t \in \Delta_{K \times K}$,  for any estimated preference matrix $\hat{f}$ if we can show that:
\begin{align*}
	\min_{\p_t \in \Delta_{K \times K}} \max_{f^\star \in \D_{\zs}} \max_{\q \in \Delta_K} & \frac{1}{2} \EE_{a^\star \sim \q, (a_t,b_t) \sim \p_t} \sbr{ f^\star[a^\star ,a_t] + f^\star[a^\star,b_t] }\\
	& - \frac{\gamma}{4} \EE_{(a_t,b_t) \sim \p_t} (\widehat{f}[a_t,b_t]- f^\star[a_t,b_t])^2 \leq \frac{\textrm{poly}(K)}{\gamma},
\end{align*}
where $D_{\zs} = \{\delta \in [-1,1]^{K \times K} \mid \delta_{ij} = -\delta_{ji}, ~\forall i \neq j\}$, then given our estimates $\widehat{f} =
\widehat{f}(x_t)$ we can deploy that choice of argmin $\p_t$ per round $t$. The  above inequality would then imply:
\begin{align}
	\label{eq:mm3}
	\nonumber \breg_T & \leq \frac{\gamma}{4} \sum_{t=1}^T \EE_{(a_t,b_t) \sim P_t}\sbr{ \rbr{ \hat{f}_t(x_t)[a_t,b_t]- f^\star(x_t)[a_t,b_t] }^2 } + \frac{\textrm{poly}(K)T}{\gamma}\\
	& \le \frac{\gamma}{4}\regsq(T) + \frac{\textrm{poly}(K)T}{\gamma} = \sqrt{\textrm{poly}(K)T\regsq(T)},
\end{align}
where the second last inequality follows from Assumption \ref{assump:oreg} and Eqn. \eqref{eq:oreg} and the last equality simply by setting the tunable parameter $\gamma = \sqrt{\frac{\textrm{poly}(K)T}{\regsq(T)}}$. 
Thus, we get an $O(\sqrt{T})$ type regret guarantee if we have access to some online regression oracle \oreg\, with 
$\regsq(T) = O(\log(T))$ square loss regret. We give some such specific examples in Cor. \ref{cor:minmax}.

Drawing inspiration from the above idea, we first define the following minmax value which analyzes a `squared-loss regulated the per round instantaneous regret' of the game:

\begin{align}
\label{eq:Vgam}
V(\gamma):= \min_{\p \in \Delta_{K \times K}} \max_{f^* \in D_{\zs}} \max_{i^* \in [K]} \bigg[~\sum_{k=1}^{K}f^*(i^*,k)\frac{p^\ell[k] + p^r[k]}{2} - \frac{\gamma}{4}\sum_{i \neq j}p[i,j]\big( f^\star_{ij} - \hf_{ij} \big)^2\bigg]
\end{align}
where $\p_t^{\ell}$ and $\p_t^{r}$ respectively denotes the marginal distribution of the left arm $a_t$ and right arm $b_t$ when drawn according to $(a_t,b_t) \sim \p_t$, $\gamma > 0$ is some tunable parameter to be specified later. 
%For any $f \in D_{\zs}$, and $k \in [K]$, we also define $f(*,k) = \max_{i \in [K]}f(i,k)$.
The following lemma shows the above minmax value $V(\gamma)$ is bounded at every round $t$. 

\begin{restatable}[]{lem}{lemmm}
	\label{lem:minmax}
For any $\gamma > 13K/8$, $V(\gamma) \le \frac{K}{\gamma}$.
\end{restatable}

\begin{proof}[Sketch of Lem. \ref{lem:minmax}]
	Note $V(\gamma)$ can be equivalently written as:
	
	\begin{align}
		\label{eq:mm1}
		\nonumber V(\gamma) = & \min_{\p \in \Delta_{K\times K}} \max_{i^\star  \in [K]} \max_{f \in D_{\zs}} ~\sum_{k=1}^{K}f(i^\star ,k)\frac{p^\ell[k] + p^r[k]}{2} - \frac{\gamma}{4}\sum_{i \neq j}p[i,j]\big( f_{ij} - \hf_{ij} \big)^2\\
		& \implies \min_{\p \in \Delta_{K\times K}} \max_{i^\star   \in [K]} \max_{\delta \in D_{\zs}}~\sum_{k=1}^{K}[\hf(i^\star  ,k) + \delta_{i^\star  k}]\frac{p^\ell[k] + p^r[k]}{2} - \sum_{i \neq j}\frac{\gamma}{4}p[i,j]\delta_{ij}^2
	\end{align}
	
	Now given any fixed $\p \in \Delta_{K\times K}$ and $i^\star   \in [K]$, optimizing w.r.t. ${\delta \in D_\zs}$ one can obtain:
	
	\begin{align*}
		\nonumber V&(\gamma) = \min_{\p \in \Delta_{K \times K}} \max_{i^\star   \in [K]} ~\sum_{k=1}^{K}\hf(i^\star  ,k) \frac{p^\ell[k] + p^r[k]}{2} + \frac{3}{16}\sum_{k=1}^K\frac{(p^\ell[k] + p^r[k])^2}{4 \gamma (p[i^\star, k]+p[k,i^\star])} \\
		\nonumber	& \overset{(1)}{\le} \min_{\p \in \Delta_{K}} \max_{i^\star   \in [K]} ~\sum_{k=1}^{K}\hf(i^\star  ,k) p[k] + \frac{3}{32}\sum_{k=1}^K\frac{p[k]}{\gamma p[i^\star]} = \min_{\p \in \Delta_{K}} \max_{\q \in \Delta_K} \q\hf\p + \frac{3}{32 \gamma}\sum_{a=1}^{K} \frac{q[a]}{p[a]},
		%\label{eq:mm2}
	\end{align*}
	where $(1)$ holds if we consider $\p \in \Delta_{K \times K}$ to be a product distribution, s.t. $p[a,b] = p[a] p[b], ~\forall a,b, \in [K]$. Thus $\p^\ell[k] = \p^\ell[k], ~\forall k \in [K]$. 
	Defining $\p^{(\epsilon)}:= (1-\epsilon)\p + \epsilon \mathbf{1}/K$, $\forall \p \in\Delta_K$, note:
	
	\begin{align*}
		& \min_{\p \in \Delta_K} \max_{\q \in \Delta_K} \q^\top \hf \p + \frac{3}{32\gamma} \sum_{a=1}^K \frac{q[a]}{p[a]}
		\leq \min_{\p \in \Delta_K} \max_{\q \in \Delta_K} \q^\top \hat{f}\p^{(\epsilon)} + \frac{3}{32\gamma}\sum_{a=1}^K \frac{q[a]}{p^{(\epsilon)}[a]}
	\end{align*}
	Now we can apply the minimax swap, since the objective is defined everywhere (as long as $\epsilon > 0$), convex in $\p$ and linear in $\q$. Doing so, we get:
	\begin{align*}
		%\label{eq:mm3}
		\nonumber \max_{\q \in \Delta_K}& \min_{\p \in \Delta_K} \q^\top \hf \p^{(\epsilon)} + \frac{3}{32\gamma}\sum_a \frac{q[a]}{p^{(\epsilon)}[a]}
		\leq \max_{\q \in \Delta_K} \q^\top \hf \q^{(\epsilon)} + \frac{3}{32\gamma} \sum_{a=1}^K \frac{q[a]}{q^{(\epsilon)}[a]}\\
		\nonumber & = \max_{\q \in \Delta_K} (1-\epsilon) \q^\top \hf \q + \epsilon \q^\top \hf \mathbf{1}/K + \frac{3}{32\gamma} \sum_{a=1}^K \frac{q[a]}{(1-\epsilon)q[a] + \epsilon/K}\\
		\nonumber & \overset{(2)}{\leq} \epsilon + \frac{3}{32\gamma} \max_{\q \in \Delta_K} \sum_{a=1}^K \frac{q[a]}{q[a]/2} \leq \epsilon + \frac{3K}{16\gamma} \le \frac{K}{\gamma}, 
	\end{align*}
	where $(2)$ holds since $\hf[a,b] = -\hf(b,a)$ which makes the first term $0$; the second term follows as $\q^\top \hf \mathbf{1}/K = \frac{1}{K}\sum_{a = 1}^{K}\sum_{b = 1}^{K}q[a]\hf[a,b] \le 1 ~(\text{since } \hf \in [-1,1]^{K \times K})$. The last inequality requires $\epsilon < 0.5$. So, we may set $\epsilon \leq \frac{13K}{16\gamma}$ as long as $\gamma > \frac{13K}{8}$. Complete proof is given in Appendix \ref{app:v_gam}.
	% then Eqn.~\pref{eq:p_main_def} is feasible as long as $\gamma > 2$. 
\end{proof}

%\begin{rem}
Noting that the first term and the second term in $V(\gamma)$ respectively correspond to the instantaneous regret of the learner at round $t$ and the squared loss of the regressor. 
Lem. \ref{lem:minmax} indicates irrespective of the choice of $i^* \in [K]$ and $f^* \in \D_{\zs}$ of the adversary, there exists a distribution over the actions $\p$, that the learner can choose to play from, such that the instantaneous regret with respect any $f^*$ would be bounded by the squared prediction error w.r.t. $f^*$ and an only an additive constant $K/\gamma$. 
%
Now, summing over all $t \in [T]$, the first term becomes the $\breg$\, over $T$ rounds which can be upper bounded by $\regsq(T)$ as argued above (see derivation of Eqn. \eqref{eq:mm3}), and simply choosing $\gamma = \sqrt{\frac{KT}{\regsq(T)}}$ we achieve a regret guarantee of $O(\sqrt{KT \regsq(T)})$. 

Precisely, at each round $t$, if the learner choose to play $(a_t,b_t) \sim \p_t$ such that $\p_t$ satisfies the bound of Lem. \ref{lem:minmax},
then we achieve $\breg_T \le \sqrt{KT \regsq(T)}$. This leads to our main theorem (see Thm. \ref{thm:minmax}). 
%
Further the choice of $\p_t$ obtain from the derivation of Lem. \ref{lem:minmax} immediately yields 
the following algorithm which is computationally efficient and near-optimal for many special function classes $\cF$ (see Rem. \ref{rem:minmax}, Cor. \ref{cor:minmax}).
The intuitive rationale behind choice of $\p_t$ in Alg. \ref{alg:genf} (Line $8$) is further elaborated in Sec. \ref{sec:simpler}. Alg. \ref{alg:genf} describes the resulting algorithm in details.
\vspace{-10pt}
\begin{center}
	\begin{algorithm}[h]
		\caption{\textbf{\algf}}
		\label{alg:genf}
		\begin{algorithmic}[1]	
			%
			\STATE {\bfseries input:} Arm set: $[K]$, parameters $\gamma > 0$. 
			\STATE ~~~~~~~~~~ $\mathcal{OR}eg$: An instance of \oreg\, for function class $\cF$
			\STATE {\bfseries init:} $\hf_{1}[a,b] = 0, ~\forall a,b \in [K]$ 
			%
			\FOR{$t = 1, 2, \ldots, T$}
			%
			\STATE Receive context $x_t$
			
			\STATE $\forall$ $a < b, \, a,b \in [K]\times [K]$: Query $\hf(x_t)[a,b] \leftarrow \mathcal{OR}eg \Big(x_t,a,b,  \{(x_\tau,a_\tau,b_\tau),y_\tau\}_{\tau = 1}^{t-1}\Big)$ 
			
			\STATE Play the duel $(a_t,b_t)$ and receive the preference feedback $o_t \sim \text{Ber}(\P_t(a_t,b_t))$
			
			\STATE Find any $\p_t$ s.t. $\forall \q \in \Delta_K: \q^\top \hat{f}_t \p_t + \frac{1}{\gamma} \sum_{a=1}^K \frac{q[a]}{p_t[a]} \leq \frac{K}{\gamma}$ 
			
			\STATE Play $a_t,b_t \overset{\text{iid}}{\sim} \p_t$ and receive the preference feedback $o_t \in \{\pm 1\}$
			
			\ENDFOR 
			%\STATE Return $\bsigma'$
		\end{algorithmic}
	\end{algorithm}
	%\vspace{2pt}
\end{center}
\vspace{-10pt}
\begin{thm}
	\label{thm:minmax}	
	Under Assumption \ref{assump:oreg}, for any $f^\star \in \cF$, \algf\, (Alg. \ref{alg:genf}) with $\gamma = \sqrt{\frac{KT}{\regsq(T)}}$ ensures: $\breg_T[\algf] \le \sqrt{KT \regsq(T)},$
	for any $T > 3 K \regsq(T)$.
\end{thm}

\noindent
Note: As Lem. \ref{lem:minmax} requires $\gamma > \frac{13K}{8}$, we need $T > 3 K \regsq(T)$ for the constraint to hold good.

Cor. \ref{cor:minmax} derives the regret bound of Alg. \ref{alg:genf} for some special realizability function classes as introduced in Rem. \ref{rem:cases} and Appendix \ref{sec:eg_oreg}. A detailed discussion can be found in Appendix \ref{app:spcl_reg}.

\begin{cor}
	\label{cor:minmax} \algf\, (Alg. \ref{alg:genf}) yields the following best-response guarantees for some structured function classes $(\cF)$:
	\hspace{1pt} \textbf{(1).} Any finite regression class $\cF$: $O(\sqrt{KT \log |\cF|})$.
	\hspace{1pt} \textbf{(2).} Class of linear predictors $O(\sqrt{d K T \log(T/d)})$.   
	\hspace{1pt} \textbf{(3).} Class of generalized linear predictors: $O\Big(\sqrt{\frac{d K T \log T}{\kappa_\sigma^2}}\Big)$.   
	\hspace{1pt} \textbf{(4).} Reproducing Kernel Hilbert Space:  $O(\sqrt{KT^{3/4}})$.
	\hspace{1pt} \textbf{(5).} Banach Space: $O(\sqrt{KD^{-1/2}T^{3/4}})$.
	%\end{enumerate}
\end{cor}


\begin{rem}[Stronger Regret Guarantee with Time-Variant Realizability ]
	\label{rem:minmax}
	The regret bound of Alg. \ref{alg:genf} (Thm. \ref{thm:minmax}) holds for a stronger definition of best-response regret where $f^\star_t \in \cF$ can be chosen arbitrarily per round $t$, as follows from the minmax guarantee of Lem. \ref{lem:minmax}. %Recalling the definition from Sec. \ref{sec:prob}, precisely, we can claim that $\wbreg_T[\algf] \le \sqrt{KT \regsq(T)}$.
	However, note this does not necessary imply a sublinear regret guarantee unless we have a \oreg\, with $o(\sqrt T)$ regret guarantee. While such an online regression oracle might not exist for any arbitrary sequence $\{f_1^*,\ldots, f_T^*\}$, for slowing varying realizable sequence, e.g. $\max_{i,j \in [K]}\max_{t \in [T-1]}|f_t^*(i,j) - f_{t+1}^*(i,j)| \leq \frac{1}{\sqrt T}$, its indeed possible to achieve low regret for any arbitrary time-variant realizability sequence. \ascomment{Please Check.}  
\end{rem}

\begin{rem}[Computation Complexity of Alg. \ref{alg:genf}]
\label{rem:comp}
Assuming access to an `efficient' \oreg, the only other computational bottleneck of \algf\, lies in computing $\p_t$ per round (Line $\#8$, Alg. \ref{alg:genf}). However this is efficiently solvable since the condition on Line $8$ can be equivalently written as: Find $\p_t$ such that $\forall a \in [K]$, $\e_a^\top \hat{f}_t \p_t + \frac{1}{\gamma} \frac{1}{p_t[a]} \leq \frac{K}{\gamma}$ which is $\textrm{poly}(K)$
 solvable by any convex programming method. Note that proof of Lem. \ref{lem:minmax} shows such a $\p_t$ always exists.
\end{rem}

%\begin{rem}[Optimality of Alg. \ref{alg:genf}]
%	That this is not optimal for lin and std case.
%\end{rem}

\subsection{Simpler Analysis of Thm. \ref{thm:minmax}}
\label{sec:simpler}

Given the choice of $\p_t$ in the derivation of Lem. \ref{lem:minmax}, we now give an {even more simpler and direct proof} for Thm. \ref{thm:minmax}. %(or more precisely Lem. \ref{lem:minmax} from which Thm. \ref{thm:minmax} follows straightforwardly). 
%
Let us first try to prove the per-round inequality of Lem. \ref{lem:minmax} more intuitively. We drop the notation subscript $t$ for convenience. We also start assuming that the dueling arms $(a,b)$ are drawn from a product measure $(a,b) \sim \p \times \p$ for some $\p \in
\Delta_K$ at each round, and lets replace the `best response' $i^* \in [K]$ of that round by the `best response distribution' $\q \in \Delta_K$ \footnote{They are equivalent in the sense the (optimal) $\arg\max \q$ vector is essentially $1$-hot since the objective is linear in $\q$.}. Then rewriting the LHS of Eqn. \eqref{eq:Vgam} in matrix-vector notation:
$
	\min_{\p \in \Delta_K} \max_{f^\star \in \Pcal} \max_{\q \in \Delta_K} \q^\top f^\star \p - \frac{\gamma}{4}\EE_{a,b\sim \p^2} (\widehat{f}[a,b] - f^\star[a,b])^2.
$
%
Now suppose we ``somehow'' (see Remark~\ref{rem:comp}) find $\p$ such that: %(\blue{@AK: Add some intuitive explanation of this weighted `q vs p' + importance sampling estimate criterion that p should satisfy?})
\begin{align}
	\forall \q \in \Delta_K: \q^\top \hat{f} \p + \frac{1}{\gamma} \sum_a \frac{q[a]}{p[a]} \leq \frac{K}{\gamma} 
	\label{eq:p_main_def}
\end{align}

Then for any $f^\star$ and any $\q$ we have:
\begin{align*}
	\q^\top f^\star \p &\leq \q^\top (f^\star - \hat{f}) \p - \frac{1}{\gamma} \sum_a \frac{q[a]}{p[a]} + \frac{K}{\gamma}\\
	& = \sum_{a=1}^K \frac{q[a]}{\sqrt{p[a] \gamma}} \cdot \sqrt{p[a]\gamma} (f^\star[a,\cdot] - \hat{f}[a,\cdot]) \p - \frac{1}{\gamma} \sum_a \frac{q[a]}{p[a]} + \frac{K}{\gamma}\\
	& = \sum_{a=1}^K \sqrt{\frac{q[a]^2}{{p[a] \gamma}} \cdot {p[a]\gamma} \big((f^\star[a,\cdot] - \hat{f}[a,\cdot]) \p\big)^2} - \frac{1}{\gamma} \sum_a \frac{q[a]}{p[a]} + \frac{K}{\gamma}\\
%
	& \leq \frac{1}{\gamma} \sum_a \frac{q[a]^2}{p[a]} + \gamma \sum_a p[a] \rbr{ (f^\star[a,\cdot] - \hat{f}[a,\cdot]) \p}^2 - \frac{1}{\gamma} \sum_a \frac{q[a]}{p[a]} + \frac{K}{\gamma}\\
	& \leq \gamma \sum_a p[a] \rbr{ (f^\star[a,\cdot] - \hat{f}[a,\cdot]) \p}^2 + \frac{K}{\gamma}\\
	& = \gamma \sum_a p[a] \rbr{ \EE_{b \sim \p} (f^\star[a,b] - \hat{f}[a,b])}^2 + \frac{K}{\gamma}\\
	& \leq \gamma \sum_{a,b} p[a]p[b] (f^\star[a,b] - \hat{f}[a,b])^2 + \frac{K}{\gamma},
\end{align*}
where the first inequality follows from AM-GM inequality: For any $x,y \in \R_+, \frac{x+y}{2} > \sqrt{xy}$.
So we can ``easily'' verify that playing this type of distribution $\p_t$ (satisfying Eqn. \eqref{eq:p_main_def}) at each round $t$, will lead to the desired regret guarantee of Thm. \ref{thm:minmax}. Start by noting that when the learner plays $(a_t,b_t)$ from a product distribution s.t. $(a_t,b_t) \sim \p_t \times \p_t$. Then the best-response regret becomes:% can be rewritten as:
\begin{align*}
\breg_T &:= \sum_{t=1}^T \max_{\q \in \Delta_K} \EE_{a \sim \q} \EE_{a_t \sim \p_t} \sbr{f^\star(x_t)[a, a_t]} = \sum_{t=1}^T \max_{\q \in \Delta_K} \q^\top f^\star \p_t\\
& \leq \Big[ \gamma\regsq(T) + \sum_{t=1}^T (K/\gamma)  \Big] = \sqrt{KT \regsq(T)}
\end{align*} 
where the last inequality follows from the derivation and Eqn.  \eqref{eq:oreg}) and last equality is due to choosing $\gamma = \sqrt{\frac{KT}{\regsq(T)}}$, which leads to the desired regret guarantee of Thm. \ref{thm:minmax}. 

\iffalse%%%%%%%%%%%%%%%%%%%%%%%%
Let us now try to verify that~\pref{eq:p_main_def} can roughly hold. To do this, let us first mix $\p$ with a little bit of uniform distribution. For any $\p$, let $\p_{\epsilon} = (1-\epsilon)\p + \epsilon \mathbf{1}/K$. Then
\begin{align*}
	& \min_{\p \in \Delta_K} \max_{\q} \q^\top \hat{f} \p + \frac{1}{\gamma} \sum_a \frac{q[a]}{p[a]}
	\leq \min_{\p \in \Delta_K} \max_{\q} \q^\top \hat{f} p_{\epsilon} + \frac{1}{\gamma}\sum_a \frac{q[a]}{p_{\epsilon}[a]}
\end{align*}
Now we can apply the minimax swap, since the objective is defined everywhere (this requires $\epsilon > 0$), convex in $\p$ and linear in $\q$. Doing so, we get
\begin{align*}
	= \max_q \min_p \q^\top \hat{f} p_{\epsilon} + \frac{1}{\gamma}\sum_a \frac{q[a]}{p_{\epsilon}[a]}
	& \leq \max_q \q^\top \hat{f} q_\epsilon + \frac{1}{\gamma} \sum_a \frac{q[a]}{q_\epsilon[a]}\\
	& \leq \max_q (1-\epsilon) \q^\top \hat{f} \q + \epsilon \q^\top \hat{f} \mathbf{1}/K + \frac{1}{\gamma} \sum_a \frac{q[a]}{(1-\epsilon)q[a] + \epsilon/K}\\
	& \leq \epsilon + \frac{1}{\gamma} \max_q \sum_a \frac{q[a]}{q[a]/2} \leq \epsilon + \frac{2A}{\gamma} 
\end{align*}
Here for the last inequality we require that $\epsilon < 1/2$. So, if we set $\epsilon = 1/\gamma$ then~\pref{eq:p_main_def} is feasible.
\fi %%%%%%%%%%%%%%%%%%%%%%%%%%%


==> linf.tex <==
\section{Warm Up: Structured Function Classes}
\label{sec:linf}

We start with the setup of standard $K$-armed dueling bandits where the context set is singleton ($|\cX|=1$) or $f^\star$ is a constant mapping (independent of the context) such that $f(x_t) = \P \in [-1,1]^{K \times K}$ for some fixed (and unknown) pairwise preference matrix $\P$. We denote this setup as \stdb\, in brief. 
Thus in this case, the concept of best-response regret simply becomes the regret of learner's action sequence $\{(a_t,b_t)\}_{t \in [T]}$ w.r.t. the best competitor policies $\q_t \in \Delta_K$ for the fixed underlying preference matrix $\P$ the at each round:

\begin{align}
	\label{eq:breg_std}
	\mathrm{StdDB(K)}\mbox{-}\mathrm{BR}\mbox{-}\mathrm{Regret(P)}_T := \sum_{t=1}^T \max_{q_t \in \Delta_K} \EE_{a \sim \q_t} \EE_{(a_t,b_t) \sim \p_t} \frac{\sbr{P[a, a_t] + P[a,b_t]}}{2}
\end{align}


 The motivation of this section is to show how we can borrow techniques from two-player Markov games literature (e.g. see Alg. $1$ in \cite{bai+20}) to achieve optimal (instance independent) $\tO(K\sqrt{T})$ type `best-response' regret guarantees for standard $K$-armed dueling bandits. The problem was not studied in the existing dueling bandit literature in this particular form of regret, as motivated in Sec. \ref{sec:rel}. We are the first to incorporate the ideas from Markov games based RL, precisely the idea of using coarse correlated equilibrium (CCE), to yield efficient and optimal algorithms (Alg. \ref{alg:stdb}) for standard $K$-armed dueling bandits on best-response $\breg$.
%
%In particular, our Alg. \ref{alg:genf} is shown to yield $\tO(\sqrt{KT})$ regret which is provably optimal (Thm. \ref{thm:stdk}, Rem. \ref{rem:stdk}). 

%\ascomment{repeat: can be removed} Recall, our studied notion of regret is stronger than the regret definition used standard dueling bandit literature as the later just evaluates the learner's action sequence against a fixed `good-strategy' whereas we  evaluate the learner's individual action at each round $t$, $\{(a_t,b_t)\}$, dynamically against it's `toughest-challenger' $\q_t \in \Delta_K$ at that round, which is hence a much stricter notion of regret to optimize on (see discussions in Sec. \ref{sec:rel}).
%
Moreover our proposed algorithm \algc\, can be easily extended to any {statistical estimation based UCB type algorithms}, e.g. to the setting of linear realizable function class (Thm. \ref{thm:linf}), or even generalized linear function classes, etc (Sec. \ref{sec:linf_o}). 

%In this case we assume each item pair is represented by a linear feature $\x_{ab} \in \R^d$, and $\cF:= \{ f_\w \mid f_\w(\x)[a,b] = \x_{ab}^\top \w, \forall \x \}$s

\subsection{\algc: Algorithm and Analysis for \stdb}

\textbf{Main Ideas: } In one words algorithm tries to find the Nash Equilibrium strategy of $\P$ and play according to that, which would of course lead to $0$ per round best-regret had it been possible. But since $\P$ is unknown, it tries to estimate $\P$ by maintaining the empirical pairwise preference entries $\hP_{ij}(t)$ for each pair $(i,j) \in [K]\times [K]$, at each round $t$. Note $\boldsymbol{\hP}(t)$ also a zero-sum matrix by definition. Now given $\boldsymbol{\hP}(t)$, it computes an upper confidence matrix $\U(t)$ of $\boldsymbol{\hP}(t)$, defining $U_{ij}(t):= \hP_{ij}(t) + O\bigg(\sqrt{\frac{\log{K T}}{n_{ij}(t)} }\bigg)$ and finds a Coarse-Correlated Equilibrium (CCE), say $\p_t \in \Delta_{K \times K}$ of the `general sum game matrix' $U(t)$, which is defined to be a joint distribution over the action-profile of the players such that 
no player has incentive in deviating from their own strategy (as per $\p_t$) unilaterally assuming no player has access to the other player's actions \citep{pdbook}. 
See Eqn. \eqref{eq:cce} for the formal CCE definition in our setup. 
Note a CCE strategy is guaranteed to exist for any finite general-sum matrix and efficiently computable using linear programming \citep{bai+20,pdbook}.
Upon computing $\p_t$, the learner simply plays $(a_t,b_t)\sim \p_t$ and updates the empirical preference estimate $\hP_{a_t b_t}(t+1)$ according to the dueling outcome $o_t$. The algorithm is detailed Alg. \ref{alg:stdb}. 
 

%\textbf{Two player zero sum game $G$.} For any pair of actions $(i,j)$, the row and the column player's value is say $U_{ij}$ and $v_{ij}$ such that $U_{ij} = -v_{ij}$, ~$\forall i \neq j$. 

%\textbf{Preference matrix $(\P)$ as a zero sum game.} Note $p_{ij} = 1-p_{ji}$. Define row player's value as $U_{ij} = 2p_{ij} - 1 \in [-1,1]$ for all $i,j \in [K]$. Thus $U_{ij} = 2p_{ij} - 1 = 2(1-p_{ji}) - 1 = -(2p_{ji}-1) = -U_{ji}$  So $v_{ij} = -U_{ij} = U_{ji} = 2p_{ji}-1$.
\vspace{-10pt}
\begin{center}
	\begin{algorithm}[h]
		\caption{\textbf{\algc}}
		\label{alg:stdb}
		\begin{algorithmic}[1]	
			%
			\STATE {\bfseries input:} Arm set: $[K]$, parameters $\delta \in (0,1)$
			\STATE {\bfseries init:} $w_{ij}(1) \leftarrow 0$,  $\forall i,j \in [K]$. Use $n_{ij}(t) := w_{ij}(t) + w_{ji}(t) \, \forall t \in [T]$ 
			%
			\FOR{$t = 1, 2, \ldots, T$}
			%
			\STATE $\tilde P_{ij}(t) := \frac{w_{ij}(t)}{n_{ij}(t)}, \, \hP_{ij}(t):= 2\tilde P_{ij}(t)-1$, $C_{ij}(t) \leftarrow \sqrt{\frac{\log{K^2 t^2/\delta}}{n_{ij}(t)} }, ~\forall i,j \in [K]$ ~\big(we assume $\nicefrac{x}{0}:=0.5, ~\forall x \in \R$\big)
			
			\STATE $U_{ij}(t) \leftarrow \hP_{ij}(t) + C_{ij}(t)$, $U_{ii}(t) \leftarrow 0,~~\forall i, j \in [K]$  
			
			%\STATE Suppose $\cC_t:= \{ \u \in \Delta_K \mid  \big[\min_{\e_i \in \Delta_K} \u^\top \U\e_i  > 0 \big] \}$, 
			
			%\STATE Select $(\U_t,\v_t):= \arg\max_{\u, \v \in \cC_t}\u^\top \C^t\v$
			
			\STATE Denoting $\p_t^\ell(\cdot):= \sum_{b = 1}^Kp_t(\cdot,b)$ and $\p_t^r(\cdot):=\sum_{a = 1}^Kp_t(a,\cdot)$, find a policy $\p_t \in \Delta_{K \times K}$ (CCE of $U(t)$) such that:  
			\vspace{-20pt}
			\iffalse%%%%%%%%%%%%%%%%%%%%%%
			\begin{align*}
				& \sum_{a,b \in [K]^2}\p_t(a,b) [U_{a,b}(t)] \geq \max_{\pi^\star \in \Delta_{K}}\E_{a^\star \sim \pi^\star}\Big[\sum_{b \in [K]}\p_t^r(b) [U_{a^\star,b}(t)]\Big] = \max_{a^\star \in [K]}\Big[\sum_{b \in [K]}\p_t^r(b) [U_{a^\star,b}(t)]\Big]\\
				& \sum_{a,b \in [K]^2}\p_t(a,b) [\bar v_{a,b}(t)] \leq \min_{\pi^\star \in \Delta_{K}}\E_{b^\star \sim \pi^\star}\Big[\sum_{a \in [K]}\p_t^\ell(a) [\bar v_{a,b^\star}(t)]\Big] = \min_{b^\star \in [K]}\Big[\sum_{a \in [K]}\p_t^\ell(a) [\bar v_{a,b^\star}(t)]\Big]\\
			\end{align*}
			
			i.e. equivalently,
			\fi%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			
			\begin{align}
				\label{eq:cce}
				\nonumber & \sum_{a,b \in [K]\times [K]}\p_t(a,b) U_{a,b}(t) \geq \max_{a^\star \in [K]}\Big[\sum_{b \in [K]}\p_t^r(b) U_{a^\star,b}(t)\Big]\\
				&\sum_{a,b \in [K]\times [K]}\p_t(a,b) U_{b,a}(t) \geq \max_{b^\star \in [K]}\Big[\sum_{a \in [K]}\p_t^\ell(a) U_{b^\star,a}(t)\Big],
			\end{align}
			 %respectively denotes the marginal distribution of the left and the right arm for the joint distribution $\p_t$ 
			\vspace{-20pt}
			\STATE Play $(a_t,b_t) \sim \p_t$ %such that $a_t \sim \U_t,\, b_t \sim \v_t$. 
			
			\STATE Receive preference feedback $o_t \in \{-1,1\}$. $\tilde o_t \leftarrow (o_t + 1)/2$  
			\STATE Update $w_{a_t b_t}(t+1) \leftarrow w_{a_t b_t}(t) + \tilde o_t$, $w_{b_t a_t}(t+1) \leftarrow w_{b_t a_t}(t) + (1-\tilde o_t)$
			\ENDFOR 
			%\STATE Return $\bsigma'$
		\end{algorithmic}
	\end{algorithm}
	%\vspace{2pt}
\end{center}
\vspace{-20pt}

\subsubsection{Regret Analysis}
%\textbf{Claim 1.} $\C^t$ is symmetric and hence $\u^\top \C^t \v = \v^\top \C^t \u$ for all $\u,\v \in \Delta_K$.
This section analyzes the regret guarantee of Alg. \ref{alg:stdb} as claimed in Thm. \ref{thm:stdk}:

\begin{restatable}[Expected regret of \algc\, on \stdb]{thm}{thmstdb}
	\label{thm:stdk}
For the setting of standard $K$-armed dueling bandit (\stdb), the best-response regret of \algc\, (Alg. \ref{alg:stdb}) satisfies:
\begin{align*}
\mathrm{StdDB(K)}\mbox{-}\mathrm{BR}\mbox{-}\mathrm{Regret(P)}_T \le O(K\log (KT)\sqrt{T}).
\end{align*} 
\end{restatable}

\begin{rem}
	\label{rem:stdk}
	The regret bound of above algorithm is optimal in $T$ (upto logarithmic factors) as the the worst case lower bound of \stdb\, setting is known to be $\Omega(\sqrt{T})$ even with the simplistic assumption of existence of Condorcet Winner in $P$ \citep{Komiyama+15,CDB}. 
\end{rem}

\begin{proof}[Proof sketch of Thm. \ref{thm:stdk}]
The proof relies on two main results: Confidence bounding $P$ through $C(t)$ (Lem. \ref{lem:conf}), and analyzing the instantaneous regret of the column and the row player (Lem. \ref{lem:rowreg}). 
%
The first one (Lem. \ref{lem:conf}) simply guarantees that with high probability at least $(1-1/T)$, $P$ can be captured inside $\hP(t) \pm C(t)$:% which is crucially required in the later part of the proof. 

\begin{restatable}[Confidence Bounding $P$]{lem}{lemconf} Setting $\delta = \frac{1}{T}$ in Alg. \ref{alg:stdb}, we get
	\label{lem:conf}
	$$Pr\big(  \exists t \in [T], \exists (i,j) \in [K] \times [K],~ \hP_{ij}(t) - C_{ij}(t) \leq P_{ij}(t) \leq \hP_{ij}(t) + C_{ij}(t) \big) \leq 1/T$$
\end{restatable}

Now Lem. \ref{lem:rowreg} attempts to bound the learner's instantaneous regret:% in terms of the the expected confidence bounds of played duel:

\begin{restatable}[Learner's Instantaneous Regret]{lem}{lemrowreg}
	\label{lem:rowreg}
For any $q \in \Delta_K$, and $(a_t,b_t) \sim \p_t$
$$\q^\top \P (\p_t^\ell + \p_t^r) \leq 2\sum_{(a,b) \in [K]\times [K]}p_t(a,b) C_{a,b}(t).$$
\end{restatable}

The regret bound of Alg. \ref{alg:stdb} (Thm. \ref{thm:stdk}) now follows by summing the instantaneous regret upper bound of Lem. \ref{lem:rowreg} over $t \in [T]$. Complete proof is given in Appendix \ref{app:stdb_reg}.
\end{proof}

\subsection{Other Structured Function Classes}
\label{sec:linf_o}

\algc, analyzed above, can be extended to other parametric structured function classes as well which may support a statistical estimation based techniques, such as generalized linear function classes, etc. We briefly discuss the case for the linear realizable function class here: 

\vspace{3pt}\noindent 
\textbf{Setting: Dueling-Bandits with Linear Realizability (\textrm{LinDB}$(d)$)} Consider $\cX \subseteq [-1,1]^{K\times K \times d}$, such that if $\x_t$ is the context received at time $t$ then  $f(\x_t)[a,b]:= \w^\top \x_t(a,b) \in [-1,1]$ for any pair $(a,b) \in [K] \times [K]$, for some unknown $\w \in [-1,1]^d$. Note $f(\x) \in [-1,1]^{K \times K}$ for any $\x \in \cX$. Considering the same setup of Sec. \ref{sec:prob}, the goal is to again minimize the $\breg$. We detail the algorithm in Appendix \ref{app:linf} (see \algl, Alg. \ref{alg:linf}) which respects the following guarantee:
 
\begin{restatable}[Expected regret for \textrm{LinDB}]{thm}{thmlinf}
	\label{thm:linf}
	For the setting of dueling bandits with linear-realizability \textrm{LinDB}$(d)$ class, we have
	$\mathrm{LinDB}\mbox{-}\mathrm{BR}\mbox{-}\mathrm{Regret}(f^\star)_T \le O(d\log (KT)\sqrt{T}).$ 
\end{restatable}




